LMPIT-inspired Tests for Detecting a Cyclostationary Signal in Noise with Spatio-Temporal Structure

In spectrum sensing for cognitive radio, the presence of a primary user can be detected by making use of the cyclostationarity property of digital communication signals. For the general scenario of a cyclostationary signal in temporally colored and spatially correlated noise, it has previously been shown that an asymptotic generalized likelihood ratio test (GLRT) and locally most powerful invariant test (LMPIT) exist. In this paper, we derive detectors for the presence of a cyclostationary signal in various scenarios with structured noise. In particular, we consider noise that is temporally white and/or spatially uncorrelated. Detectors that make use of this additional information about the noise process have enhanced performance. We have previously derived GLRTs for these specific scenarios; here, we examine the existence of LMPITs. We show that these exist only for detecting the presence of a cyclostationary signal in spatially uncorrelated noise. For white noise, an LMPIT does not exist. Instead, we propose tests that approximate the LMPIT, and they are shown to perform well in simulations. Finally, if the noise structure is not known in advance, we also present hypothesis tests using our framework.

==> biographies.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height =1.25in,clip,keepaspectratio]{Pries}}]{Aaron Pries} (S'15)
received the M.Sc. degree in electrical engineering in 2015 from Paderborn University. He is currently a Ph.D. candidate at the Signal and System Theory Group of Paderborn University. His research interests include wireless communications and machine learning for computer vision.
\end{IEEEbiography}
%
\vspace{-5cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height =1.25in,clip,keepaspectratio]{Ramirez}}]{David Ram{\'\i}rez} (S'07-M'12-SM'16)
	received the Telecommunication Engineer degree and the Ph.D. degree in Electrical Engineering from the University of Cantabria, Spain, in 2006 and 2011, respectively. From 2006 to 2011, he was with the Communications Engineering Department, University of Cantabria, Spain. In 2011, he joined as a research associate the University of Paderborn, Germany, and later on, he became assistant professor (Akademischer Rat). He is now assistant professor (profesor visitante) with the University Carlos III of Madrid. Dr. Ram{\'\i}rez has been a visiting researcher at the University of Newcastle, Australia and at the University College London. His current research interests include signal processing for wireless communications, statistical signal processing, change-point management, and signal processing on graphs. Dr. Ram{\'\i}rez has been involved in several national and international research projects on these topics. He was the recipient of the 2012 IEEE Signal Processing Society Young Author Best Paper Award and the 2013 extraordinary Ph.D. award of the University of Cantabria. Moreover, he currently serves as associate editor for the {\em IEEE Transactions on Signal Processing} and for Signals. Finally, Dr. Ram{\'\i}rez is a member of the IEEE Technical Committee on Signal Processing Theory and Methods and was Publications Chair of the 2018 IEEE Workshop on Statistical Signal Processing.
\end{IEEEbiography}
%
\vspace{-5cm}
\begin{IEEEbiography}[{\includegraphics[width=1in,height =1.25in,clip,keepaspectratio]{PJS}}]{Peter J. Schreier} (S’03–M’04–SM’09)
was born in Munich, Germany, in 1975. He received a Master of Science from the University of Notre Dame, IN, USA, in 1999, and a Ph.D. from the University of Colorado at Boulder, CO, USA, in 2003, both in electrical engineering. From 2004 until 2011, he was on the faculty of the School of Electrical Engineering and Computer Science at the University of Newcastle, NSW, Australia. Since 2011, he has been Chaired Professor of Signal and System Theory at Paderborn University, Germany. He has spent sabbatical semesters at the University of Hawaii at Manoa, Honolulu, HI, and Colorado State University, Ft. Collins, CO.%
From 2008 until 2012, he was an Associate Editor of the {\em IEEE Transactions on Signal Processing}, and from 2010 until 2014 a Senior Area Editor for the same Transactions. Currently, he serves as an Associate Editor for the {\em IEEE Signal Processing Letters}. From 2009 until 2014, he was a member of the IEEE Technical Committee on Machine Learning for Signal Processing, and he is currently a member of the IEEE Technical Committee on Signal Processing Theory and Methods. He was the General Chair of the 2018 IEEE Statistical Signal Processing Workshop in Freiburg, Germany.
\end{IEEEbiography}


% You can push biographies down or up by placing
% a \vfill before or after them. The appropriate
% use of \vfill depends on what kind of text is
% on the last page and whether or not the columns
% are being equalized.

%\vfill

% Can be used to pull up biographies so that the bottom of the last one
% is flush with the other column.
%\enlargethispage{-5in}\\

